Mission Design of DESTINY+: Toward Active Asteroid (3200) Phaethon and Multiple Small Bodies

DESTINY+ is an upcoming JAXA Epsilon medium-class mission to fly by the Geminids meteor shower parent body (3200) Phaethon. It will be the world's first spacecraft to escape from a near-geostationary transfer orbit into deep space using a low-thrust propulsion system. In doing so, DESTINY+ will demonstrate a number of technologies that include a highly efficient ion engine system, lightweight solar array panels, and advanced asteroid flyby observation instruments. These demonstrations will pave the way for JAXA's envisioned low-cost, high-frequency space exploration plans. Following the Phaethon flyby observation, DESTINY+ will visit additional asteroids as its extended mission. The mission design is divided into three phases: a spiral-shaped apogee-raising phase, a multi-lunar-flyby phase to escape Earth, and an interplanetary and asteroids flyby phase. The main challenges include the optimization of the many-revolution low-thrust spiral phase under operational constraints; the design of a multi-lunar-flyby sequence in a multi-body environment; and the design of multiple asteroid flybys connected via Earth gravity assists. This paper shows a novel, practical approach to tackle these complex problems, and presents feasible solutions found within the mass budget and mission constraints. Among them, the baseline solution is shown and discussed in depth; DESTINY+ will spend two years raising its apogee with ion engines, followed by four lunar gravity assists, and a flyby of asteroids (3200) Phaethon and (155140) 2005 UD. Finally, the flight operations plan for the spiral phase and the asteroid flyby phase are presented in detail.

==> contents/abbreviations.tex <==
% This packagae is used to make list of symbols and list of abbreviations at the start of the report. 
% \makeglossaries
% This is the syntax for the symbol 
% \newglossaryentry{here comes the command you will use}
% {
%         name=here comes the symbol,
%         description={Is a mark up language specially suited for 
% scientific documents}
% }
% This is the syntax for abbreviations 
% \newacronym{here comes the command you will use}{here comes the abbereviation}{here comes the full form of the abbreviation}

% These are the commands to be used in the text:
% For the symbol  
% \gls{here comes the command you will use} -->  first letter small 
% \Gls{here comes the command you will use} -->  first letter caps
% \glspl{here comes the command you will use} -->  first letter small and plural 
% \Glspl{here comes the command you will use} -->  first letter caps and plural 

% For the abbreviations: 
% \acrshort{here comes the command you will use} -> will use the abbreviation 
% \acrlong{here comes the command you will use} -> will use the full form 
% \acrfull{here comes the command you will use} -> will use the full form (abbreviation).  

%\newacronym{test}{TEST}{This section is not numbered. A nomenclature section could be provided when there are mathematical symbols in your paper. Superscripts and subscripts must be listed separately. Nomenclature definitions should not appear again in the text.}

%\newglossaryentry{test_symbol}
%{
%        name=$\theta_{test}$, 
%        description={This section is not numbered. Define acronyms and abbreviations that are not standard in this section. Such acronyms and abbreviations that are unavoidable in the abstract must be defined at their first mention there. Ensure consistency of abbreviations throughout the article. Always use the full title followed by the acronym (abbreviation) to be used, e.g., reusable suborbital launch vehicle (RSLV), International Space Station (ISS).}
%}

% \newacronym{destiny}{DESTINY$^+$}{Demonstration and Experiment of Space Technology and INterplanetary voYage, Phaethon fLyby and dUSt analysis}
